Generalization in quasi-periodic environments

By and large the behavior of stochastic gradient is regarded as a challenging problem, and it is often presented in the framework of statistical machine learning. This paper offers a novel view on the analysis of on-line models of learning that arises when dealing with a generalized version of stochastic gradient that is based on dissipative dynamics. In order to face the complex evolution of these models, a systematic treatment is proposed which is based on energy balance equations that are derived by means of the Caldirola-Kanai (CK) Hamiltonian. According to these equations, learning can be regarded as an ordering process which corresponds with the decrement of the loss function. Finally, the main results established in this paper is that in the case of quasi-periodic environments, where the pattern novelty is progressively limited as time goes by, the system dynamics yields an asymptotically consistent solution in the weight space, that is the solution maps similar patterns to the same decision.

==> mydefs.tex <==

% For et al.'ing things
\newcommand{\etal}{{\em et al.\/}}
\def\annote#1{\par {\bf #1}\par}


%\def\NaturalSet{\mbox{I\hspace*{-0.16em}N}}
\def\RealSet{\mbox{I\hspace*{-0.16em}R}}
\def\R{\mathbb{R}} %the set of real numbers
\def\Reals{\mathbb{R}} %the set of real numbers
\def\Nat{\mathbb{N}}% set of natural numbers
\def\Nn{\mathbb{N}}
\def\Qn{\mathbb{Q}}
\def\scrE{\mathscr{E}}
\def\X{\mathscr{X}}
\def\Y{\mathscr{Y}}
\def\Z{\mathscr{Z}}

\def\T{\mathscr{T}}

\font\mathlet=eurm10 
\def\eff{\hbox{\mathlet f}}
\def\Vi{\hbox{\mathlet V}}
\def\bud{\mathtt{nil}}

\def\NaturalSet{\mbox{$I\!\! N$}}
%\def\RealSet{\mbox{$I\!\!R$}}
%\def\func#1{\mbox{$#1(\cdot)$}}

\def\N{\mbox{$I\!\! N$}}
\def\R{\mbox{$I\!\!R$}}
\def\C{\mbox{\rm C}}

\def\QED{\protect{\flushright{$\Box$}}}
%\def\QED{\mbox{\rule[0pt]{1.5ex}{1.5ex}}}
%\def\qed{\hspace*{\fill}~\protect{\QED}}
%\def\ONE{\Huge{\bf 1}\hspace{-.1cm}\normalsize{\mbox {\bf I}}}
%\def\ONE{{\bf 1}\hspace{-.3cm}{\mbox {\bf I}}}
\def\ONES{\mbox{\unboldmath $1$}}
%\def\ONES{\mbox{\unboldmath 1} \hspace{-.1cm}\normalsize{\mbox {\unboldmath I}}}
\def\ZERO{\bf 0}

\def\sequence#1#2#3{#1^{#3\choose #2}}
\def\chain{\oplus}
\def\quantize#1{\ulcorner #1 \lrcorner}
\def\path{\leadsto}
\def\nil{\mbox{\boldmath $0$}} 
\def\ONE{\mbox{\boldmath $1$}} 
\def\BBox{\vrule height 1.2ex width 1.2ex depth -.1ex}
\def\warp{\bowtie}
\def\RealSet{\mbox{$I\!\!R$}}


\def\smap{F}
\def\gmap{\mbox{\Large{$\tau$}}}
\def\tmap{f}


\def\shape#1{\rm }
\def\ot{\overline{t}}
\def\osigma{\overline{\sigma}}
\def\Set{\mbox{$\mbox{\sc set}$}}
\def\Reset{\mbox{$\mbox{\sc reset}$}}
\def\Nil{\mbox{$\mbox{\sc nil}$}}
\def\Not{\mbox{$\mbox{\sc not}$}}
\def\False{\mbox{$\mbox{\sc false}$}}
\def\True{\mbox{$\mbox{\sc true}$}}

\def\Action{$\mbox{\boldmath ${\cal A}$}$}

\def\pa{\mbox{pa}}
\def\vert{\mbox{vert}}
\def\de{\mbox{de}}
\def\det{\mbox{det}}
\def\diag{\mbox{diag}}
\def\dim{\mbox{dim}}
\def\sign{\mbox{sign}}
\def\diag{\mbox{diag}}
\def\ln{\mbox{ln}}
%\def\arg{\mbox{\shape{n}\selectfont arg}}
\def\softmax{\mbox{softmax}}
\def\argmax{\mathop{\operator@font argmax}}
\def\argmin{\mathop{\operator@font argmin}}

\def\BA{\mbox{\boldmath $A$}}
\def\BB{\mbox{\boldmath $B$}}
\def\BC{\mbox{\boldmath $C$}}
\def\BD{\mbox{\boldmath $D$}}
\def\BG{\mbox{\boldmath $G$}}
\def\BF{\mbox{\boldmath $F$}}
\def\BI{\mbox{\boldmath $I$}} 
\def\BPhi{\mbox{\boldmath $\Phi$}}
\def\BR{\mbox{\boldmath $R$}}
\def\BS{\mbox{\boldmath $S$}} 
\def\BL{\mbox{\boldmath $L$}} 
\def\BTheta{\mbox{\boldmath $\Theta$}}
\def\Bsigma{\mbox{\boldmath $\sigma$}}
\def\BU{\mbox{\boldmath $U$}} 
\def\BH{\mbox{\boldmath $H$}} 
\def\BM{\mbox{\boldmath $M$}}
\def\BN{\mbox{\boldmath $N$}}
\def\BP{\mbox{\boldmath $P$}} 
\def\BT{\mbox{\boldmath $T$}}
\def\BV{\mbox{\boldmath $V$}} 
\def\BX{\mbox{\boldmath $X$}}
\def\BB{\mbox{\boldmath $B$}}
\def\BC{\mbox{\boldmath $C$}}
\def\BR{\mbox{\boldmath $R$}}
\def\BY{\mbox{\boldmath $Y$}} 
\def\BW{\mbox{\boldmath $W$}}
\def\BZ{\mbox{\boldmath $Z$}}
\def\B0{\mbox{\boldmath $0$}}
\def\Balpha{\mbox{\boldmath $\alpha$}}
\def\Ba{\mbox{\boldmath $a$}}
\def\Bbeta{\mbox{\boldmath $\beta$}}
\def\Bb{\mbox{\boldmath $b$}}
\def\Bc{\mbox{\boldmath $c$}}
\def\Bd{\mbox{\boldmath $b$}}
\def\Bgamma{\mbox{\boldmath $\gamma$}}
\def\Bdelta{\mbox{\boldmath $\delta$}}
\def\BDelta{\mbox{\boldmath $\Delta$}}
\def\Beta{\mbox{\boldmath $\eta$}}
\def\Be{\mbox{\boldmath $e$}}
\def\Bepsilon{\mbox{\boldmath $\epsilon$}}
\def\Bf{\mbox{\boldmath $f$}}
\def\Blambda{\mbox{\boldmath $\lambda$}}
\def\Bg{\mbox{\boldmath $g$}}
\def\Bmu{\mbox{\boldmath $\mu$}} 
\def\Bnu{\mbox{\boldmath $\nu$}} 
\def\Bm{\mbox{\boldmath $m$}}
\def\Bo{\mbox{\boldmath $o$}}
\def\Bphi{\mbox{\boldmath $\phi$}}
\def\Bpi{\mbox{\boldmath $\pi$}}
\def\Bpsi{\mbox{\boldmath $\psi$}}
\def\Bpi{\mbox{\boldmath $\pi$}}
\def\Bp{\mbox{\boldmath $p$}}
\def\Bq{\mbox{\boldmath $q$}}
\def\Br{\mbox{\boldmath $r$}}
\def\Bs{\mbox{\boldmath $s$}}
\def\Btheta{\mbox{\boldmath $\theta$}}
\def\Bdelta{\mbox{\boldmath $\delta$}}
\def\Bomega{\mbox{\boldmath $\omega$}}
\def\Bu{\mbox{\boldmath $u$}}
\def\Bvarphi{\mbox{\boldmath $\varphi$}}
\def\Bvartheta{\mbox{\boldmath $\vartheta$}}
\def\Bvarsigma{\mbox{\boldmath $\varsigma$}}
\def\Bv{\mbox{\boldmath $v$}}
\def\Bw{\mbox{\boldmath $w$}} 
\def\Bxi{\mbox{\boldmath $\xi$}}
\def\Bx{\mbox{\boldmath $x$}}
\def\Bd{\mbox{\boldmath $d$}}
\def\By{\mbox{\boldmath $y$}} 
\def\Bzeta{\mbox{\boldmath $\zeta$}}
\def\Bz{\mbox{\boldmath $z$}}
\def\EQ{\!=\!}
\def\Given{\mbox{$\: \bigl | \bigr. \:$}}
\def\MAX{\mbox{\sc max}}
\def\MIN{\mbox{\sc min}}
\def\cond{\mbox{$\chi$}}
\def\Overq{{\overline{q}}}
\def\Pr{\mbox{P}}
\def\given{\mbox{$\: | \:$}}

\def\vectw#1#2{\!\left[\!\!\begin{array}{r}#1\\#2\end{array}\!\!\right]\!}

\def\ivector#1{\sfmath{I}_{[#1]}}
\def\CalA{{\cal A}}
\def\CalB{{\cal B}}
\def\CalC{{\cal C}}
\def\CalD{{\cal D}}
\def\CalE{{\cal E}}
\def\CalF{{\cal F}}
\def\CalG{{\cal G}}
\def\CalH{{\cal H}}
\def\CalI{{\cal I}}
\def\CalK{{\cal K}}
\def\CalL{{\cal L}}
\def\CalM{{\cal M}}
\def\CalN{{\cal N}}
\def\CalO{{\cal O}}
\def\CalP{{\cal P}}
\def\CalQ{{\cal Q}}
\def\CalR{{\cal R}}
\def\CalS{{\cal S}}
\def\CalT{{\cal T}}
\def\CalU{{\cal U}}
\def\CalV{{\cal V}}
\def\CalW{{\cal W}}
\def\CalX{{\cal X}}
\def\CalY{{\cal Y}}
\def\CalZ{{\cal Z}}
\def\VecCalE{{\cal{\vec{E}}}}
\def\Alphabet{{\cal A}}
\def\Real{\mbox{$\mathbb{R}$}}
\def\AND{\mbox{${\cal B}_\wedge$}}
\def\OR{\mbox{${\cal B}_\vee$}}

\def\istar{\mbox{$\CalI^\star$}}
% \def\EqDef{\doteq}
\def\EqDef{\buildrel \rm def \over =}

\def\RefFig#1{Figure~\ref{#1}}
\def\RefTab#1{Table~\ref{#1}}
\def\RefEq#1{(\ref{#1})}
\def\RefEqs#1#2{(\ref{#1},\ref{#2})}
\def\RefCh#1{Chapter \ref{#1}}
\def\RefSect#1{\S~\ref{#1}}
\def\RefSec#1{\S~\ref{#1}}
\def\RefSub#1{\S~\ref{#1}}
\def\RefDef#1{Definition~\ref{#1}}
\def\RefTh#1{Theorem~\ref{#1}}
\def\RefTh#1{Conjecture~\ref{#1}}
\def\cdw#1{{\em \underline{#1}}}
\def\RealSet{\mbox{$I\! \! R$}}
\newcommand{\bbR}{{\mathbb{R}}}
\newcommand{\bbN}{{\mathbb{N}}}
\newcommand{\bbK}{{\mathbb{K}}} %I've added this line to compile hf2.tex Alessandro.

% An list-like environment that indents second, etc. lines of each item.
\newenvironment{defs}%
{\begin{list}{}{\setlength{\itemindent}{-\leftmargin}\setlength{\itemsep}{0pt}\setlength{\parsep}{0pt}}}%
{\end{list}}

% shrink and rotate everything for a two-pages on 1 printing using dvips.
%\input reduce.tex

% ``\heading'' is like a subsubsubsection, and takes a single argument.
% \newcommand{\heading}[1]{ \medskip
%         {\setlength{\parindent}{0in} \bf #1}
%         \nopagebreak
%         }

% ``\comment'' takes a single argument
\newcommand{\comment}[1]{}


% Local Variables: 
% mode: latex
% TeX-master: "main"
% End: 

